Manipulating Node Similarity Measures in Networks

Node similarity measures quantify how similar a pair of nodes are in a network. These similarity measures turn out to be an important fundamental tool for many real world applications such as link prediction in networks, recommender systems etc. An important class of similarity measures are local similarity measures. Two nodes are considered similar under local similarity measures if they have large overlap between their neighboring set of nodes. Manipulating node similarity measures via removing edges is an important problem. This type of manipulation, for example, hinders effectiveness of link prediction in terrorists networks. Fortunately, all the popular computational problems formulated around manipulating similarity measures turn out to be NP-hard. We, in this paper, provide fine grained complexity results of these problems through the lens of parameterized complexity. In particular, we show that some of these problems are fixed parameter tractable (FPT) with respect to various natural parameters whereas other problems remain intractable W[1]-hard and W[2]-hard in particular). Finally we show the effectiveness of our proposed FPT algorithms on real world datasets as well as synthetic networks generated using Barabasi-Albert and Erdos-Renyi models.

==> result_approx.tex <==
\section{Results: Approximation Algorithm}

\begin{theorem}
 For local similarity metrics, there is a polynomial time algorithm for the \ESED problem which approximates the total number of edges deleted within a factor of $2$.
\end{theorem}

\begin{proof}
 Let $(\GG,\SS,\CC,k)$ be an arbitrary instance of \ESED. For every pair $\{x,y\}\in\SS$, and for every vertex $u\in\GG$ with $\{u,x\}\in\GG$ and $\{u,y\}\in\GG$, if both $\{u,x\}\notin\CC$ and $\{u,y\}\notin\CC$, then we output \NO; otherwise we delete any one edge from $\{\{u,x\},\{u,y\}\}\cap\CC$. We claim that our algorithm removes at most $2$ times the number of edges that an optimal algorithm would remove... vertex cover type argument...
\end{proof}

The following claim follows immediately from the proof of Theorem 3.3 in \cite{Zhou:2019:ASL:3306127.3331707}.

\begin{corollary}
 Under \UGC, there does not exist any polynomial time algorithm for the \ESED problem which approximates the total number of edges deleted within a factor of $2-\eps$ for any real number $\eps>0$.
\end{corollary}


==> result_pc.tex <==
\section{Results: Parameterized Complexity}

\subsection{Parameterized Algorithms}

\begin{theorem}\label{thm:param_eliminating}
 For local similarity metrics, there exists an algorithm for the \ESED problem which runs in time $\OO(1.2738^k+km)$.
\end{theorem}

\begin{proof}
 Let $(\GG=(\VV,\EE),\SS,\CC,k)$ be an arbitrary instance of \ESED. For every pair $\{x,y\}\in\SS$ and every $u\in\VV$ with $\{\{u,x\},\{u,y\}\}\in\EE$, if $|\{\{u,x\},\{u,y\}\}\cap\CC|=0$, then we output \NO; if $|\{\{u,x\},\{u,y\}\}\cap\CC|=1$ and $k\ge1$, then we remove the edge $\{\{u,x\},\{u,y\}\}\cap\CC$ and decrease $k$ by $1$. If $\sum_{(x,y)\in \SS}{\similarity(x,y)}$ is already $0$ in the current graph, then we output \YES. Otherwise let us assume without loss of generality that the current instance be $(\GG=(\VV,\EE),\SS,\CC,k)$. Hence, for every pair $\{x,y\}\in\SS$ and every $u\in\VV$ with $\{\{u,x\},\{u,y\}\}\in\EE$, we have $\{\{u,x\},\{u,y\}\}\subseteq\CC$.
 
 We now reduce the \ESED instance to a \VC $(\GG^\pr=(\VV^\pr,\EE^\pr),k^\pr)$. We have $\VV^\pr=\{v_e: e\in\EE\}$. For any two vertices $v_{e}, v_{f}\in\VV^\pr$, we have an edge between them in $\GG^\pr$, that is $\{v_e,v_f\}\in\EE^\pr$, if there exist vertices $a,b,c\in\VV$ such that $e=\{a,b\}, f=\{b,c\},$ and $\{a,c\}\in\SS$. We also define $k^\pr=k$. We now claim that $(\GG,\SS,\CC,k)$ is a \YES instance of \ESED if and only if $(\GG^\pr,k^\pr)$ is a \YES instance of \VC.
 
 Let $(\GG,\SS,\CC,k)$ be a \YES instance of \ESED. Then there exists a subset $\FF\subseteq\EE$ of edges in \GG with $|\FF|\le k$ such that the $\sum_{(x,y)\in \SS}{\similarity(x,y)}$ is $0$ in the graph $\GG\setminus\FF$. We claim that $\WW=\{v_e: e\in\FF\}$ is a vertex cover of $\GG^\pr$. Suppose not, then there exists at least one edge $\{v_e,v_f\}\in\EE^\pr$ which \WW does not cover. Then, by the construction of $\GG^\pr$, we have three vertices $a,b,c\in\VV$ such that $e=\{a,b\}, f=\{b,c\},$ and $\{a,c\}\in\SS$. However, then we have $\similarity(a,c)>0$ and thus we have $\sum_{(x,y)\in \SS}{\similarity(x,y)}>0$ in the graph $\GG\setminus\FF$ which is a contradiction.
 
 For the other direction, let $(\GG^\pr,k^\pr)$ is a \YES instance of \VC. Then there exists a vertex cover $\WW\subseteq\VV^\pr$ of $\GG^\pr$ of size at most $k^\pr$. Let us define $\FF=\{e\in\EE: v_e\in\WW\}$. We claim that we have $\sum_{(x,y)\in \SS}{\similarity(x,y)}=0$ in the graph $\GG\setminus\FF$. Suppose not, then there exists a pair $\{a,c\}\in\SS$ such that $\similarity(a,c)>0$ in the graph $\GG\setminus\FF$. Since the similarity metric is local, there exists at least one vertex $b\in\VV$ such that we have $\{a,b\},\{b,c\}\in\EE\setminus\FF$. However, this implies that \WW does not cover the edge $\{v_{\{a,b\}}, v_{\{b,c\}}\}$ which is a contradiction.
 
 We now describe our algorithm. We first pre-process any instance $(\GG=(\VV,\EE),\SS,\CC,k)$ of \ESED and to ensure that for every pair $\{x,y\}\in\SS$ and every $u\in\VV$ with $\{\{u,x\},\{u,y\}\}\in\EE$, we have $\{\{u,x\},\{u,y\}\}\subseteq\CC$. We then construct a corresponding instance $(\GG^\pr,k^\pr)$ of \VC as described above. We then compute a vertex cover \WW (if it exists) of $(\GG^\pr,k^\pr)$ and output the corresponding set of edges of \GG to be removed. If the vertex cover instance is a \NO instance, then we output \NO. We observe that the number of vertices in the vertex cover instance is the same as the number of edges of the \ESED instance. Now the claimed running time of our algorithm follows from the fact that there is an algorithm for the \VC problem which runs in time $\OO(1.2738^k+kn)$ where $n$ is the number of vertices in the \VC instance~\cite{DBLP:conf/mfcs/ChenKX06}.
\end{proof}



\subsection{\WO-Hardness}

The following problem may be interesting for proving \WOH.

\begin{definition}[\PVC]
 Given a graph \GG and two integers $k$ and $s$, do there exist $k$ vertices which covers at least $s$ edges?
\end{definition}

We know that the \PVC problem parameterized by $k$ is \WOH.

